Modified Theories of Gravity: Traversable Wormholes

This MSc thesis is divided in to two parts. The first, covers the foundations of theories of gravitation, and, the second incorporates original work on the subject of the existence of traversable wormholes in $f(R)$ modified theories of gravity. A short incursion in the field of scalar-tensor theories had to be made, owing to an apparent inconsistency in the result previously found.

==> referenc.tex <==
%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%
\addcontentsline{toc}{chapter}{Bibliography}
% Non-BibTeX users please use
\begin {thebibliography}{99.}

















\bibitem{Guarnizo} A.~Guarnizo, {\it Variational principles in Modified Gravity: Field equations in $f(R)$
gravity}, [arXiv:gr-qc/1002.0617v1]


\bibitem{Harko:2008vy}
  T.~Harko, Z.~Kovacs and F.~S.~N.~Lobo,
  %``Electromagnetic signatures of thin accretion disks in wormhole
  %geometries,''
  Phys.\ Rev.\  D {\bf 78}, 084005 (2008);
  %[arXiv:0808.3306 [gr-qc]];
%%CITATION = ARXIV:0808.3306;%%
%
T.~Harko, Z.~Kovacs and F.~S.~N.~Lobo,
  %``Thin accretion disks in stationary axisymmetric wormhole spacetimes,''
  Phys.\ Rev.\  D {\bf 79}, 064001 (2009).
  %[arXiv:0901.3926 [gr-qc]].
  %%CITATION = PHRVA,D79,064001;%%

\bibitem{HawEll} S.~W.~Hawking \& G.~F.~R.~Ellis, {\it The Large Scale Structure of
Space-time}, (Cambridge University Press, 1973).









\bibitem{Gravitation} C.~W.~Misner, K.~S.~Thorne and  J.~A.~Wheeler, {\em Gravitation}, (W.~H.~Freeman and Co., San Francisco, 1973).


\bibitem{SSSsolution}
T. Multam\"{a}ki and I. Vilja,
%``Spherically symmetric solutions of modified field equations
%in $f(R)$ theories of gravity,''
Phys. Rev. D {\bf 74}, 064022 (2006);
%
%\bibitem{Mult2}
T. Multam\"{a}ki and I. Vilja,
%``Static and spherically symmetric
%perfect fluid solutions in $f(R)$ theories of gravity,''
[arXiv:astro-ph/0612775].
%%CITATION = ASTRO-PH 0612775;%%



\bibitem{Ohanian} H.~C.~Ohanian~\&~R. Ruffini, {\it Gravitation and Spacetime} Second Edition (W W Norton~\&~Company, 1994).
%\bibitem{Rich} Rich, {\it Fundamentals of Cosmology}



\bibitem{Pais} A.~Pais {\it ``Subtle is the Lord...'' The Science and the life of Albert Einstein}, (Cambridge University Press, 1982).

\bibitem{perlmutter}
S.~Perlmutter {\it et al.},
%``Measurements of Omega and Lambda
%from 42 High-Redshift Supernovae,''
Astrophys.\ J.\  {\bf 517}, 565 (1999).


\bibitem{riess}
A.~G.~Riess {\it et al.},
%``Observational Evidence from Supernovae for
%an Accelerating Universe and a Cosmological Constant,''
Astron.\ J.\  {\bf 116}, 1009 (1998);
Astron.\ J.\  {\bf 117}, 707 (1999).



\bibitem{schrod} E.~Sch\"{o}dinger, {\it Space-Time Structure}, (Cambridge University Press, 1950).

\bibitem{sot-PhD} T.~P.~Sotiriou {\it Modified Actions for Gravity: Theory and Phenomenology} [arXiv:gr-qc/arXiv:07c10.4438v1]




\bibitem{Stephani} H.~Stephani, {\it Relativity}, Third Edition, (Cambridge University Press, 2004).

\bibitem{Visser}
  M.~Visser,
  {\it Loretzian wormholes: from Einstein to Hawking}
  AIP Press (1995).



%\bibitem{ChapWH}
F.~S.~N.~Lobo,
  %``Chaplygin traversable wormholes,''
  Phys.\ Rev.\ {\bf D73}, 064028 (2006);
  %[arXiv:gr-qc/0511003];
  %%CITATION = PHRVA,D73,064028;%%
%
%\bibitem{vdWWH}
F.~S.~N.~Lobo,
  %``Van der Waals quintessence stars,''
  Phys.\ Rev.\  D {\bf 75}, 024023 (2007).
  %[arXiv:gr-qc/0610118].
  %%CITATION = PHRVA,D75,024023;%%



\bibitem{winberg-cos} S.~Weinberg, {\it Cosmology}, (Oxford University Press, 2008).



\end{thebibliography}
%%%%%
%\bibitem{r1}
%E.~Komatsu {\it et al.}  [WMAP Collaboration],
% arXiv:0803.0547 [astro-ph].

%\bibitem{SDSS} J. Yadav, S. Bharadwaj, B. Pandey,
%and T. R. Seshadri, Mon. Not. Roy. Astron. Soc. 364, 601 (2005)
%[astro-ph/0504315].

%\bibitem{r2}
%R.~S.~Hill {\it et al.}  [WMAP Collaboration],
% arXiv:0803.0570 [astro-ph];\\
%E.~L.~Wright {\it et al.}  [WMAP Collaboration],
% arXiv:0803.0577 [astro-ph];\\
%J.~Dunkley {\it et al.}  [WMAP Collaboration],
% arXiv:0803.0586 [astro-ph];\\
%M.~R.~Nolta {\it et al.}  [WMAP Collaboration],
% arXiv:0803.0593 [astro-ph];\\
%B.~Gold {\it et al.}  [WMAP Collaboration],
% arXiv:0803.0715 [astro-ph];\\
%G.~Hinshaw {\it et al.}  [WMAP Collaboration],
%arXiv:0803.0732
%[astro-ph].

%\bibitem{r3}
%M.~Kowalski {\it et al.} [Supernova Cosmology Project
% Collaboration], arXiv:0804.4142 [astro-ph].\\
% The numerical data of the full sample are available at
% http:$/\!/$supernova.lbl.gov/Union

%\bibitem{r4}
%D.~Rubin {\it et al.} [Supernova Cosmology Project
% Collaboration], arXiv:0807.1108 [astro-ph].

